GradTac: Spatio-Temporal Gradient Based Tactile Sensing

Tactile sensing for robotics is achieved through a variety of mechanisms, including magnetic, optical-tactile, and conductive fluid. Currently, the fluid-based sensors have struck the right balance of anthropomorphic sizes and shapes and accuracy of tactile response measurement. However, this design is plagued by a low Signal to Noise Ratio (SNR) due to the fluid based sensing mechanism "damping" the measurement values that are hard to model. To this end, we present a spatio-temporal gradient representation on the data obtained from fluid-based tactile sensors, which is inspired from neuromorphic principles of event based sensing. We present a novel algorithm (GradTac) that converts discrete data points from spatial tactile sensors into spatio-temporal surfaces and tracks tactile contours across these surfaces. Processing the tactile data using the proposed spatio-temporal domain is robust, makes it less susceptible to the inherent noise from the fluid based sensors, and allows accurate tracking of regions of touch as compared to using the raw data. We successfully evaluate and demonstrate the efficacy of GradTac on many real-world experiments performed using the Shadow Dexterous Hand, equipped with the BioTac SP sensors. Specifically, we use it for tracking tactile input across the sensor's surface, measuring relative forces, detecting linear and rotational slip, and for edge tracking. We also release an accompanying task-agnostic dataset for the BioTac SP, which we hope will provide a resource to compare and quantify various novel approaches, and motivate further research.

==> sections/conclusion.tex <==
\section{Conclusion and Future Work}
In conclusion, the work proposes a novel method to parse raw tactile data from the \btsp sensor and converts it into a spatio-temporal gradient (events) surface that closely tracks the regions of maximum tactile stimulus. Our algorithm focuses on approximating the region of touch on the skin of the \btsp sensor, which is accurate enough to perform various tactile feedback related tasks. We perform temporal aggregation on the generated events, and use that to obtain a Voronoi tesselation of the sensor's surface, which is then used to perform natural neighbors interpolation of the surface.
In comparison to other methods for tactile data processing, our method is real-time and require minimal processing overhead, at the cost of highly accurate surface deformation values.

This surface, and the resulting contours, contain information about both the location and intensity of a tactile stimulus applied to the sensor's surface. Our intermediate contour representation can then be used to perform useful tasks, related to tracking tactile stimulus across the sensor, measuring relative force, slippage detection and classification of direction, and tracking edges on a plane. We demonstrate experiments and discuss results for each.

Lastly, our approach is independent of any particular sensor type, and we present an accompanying dataset of task-agnostic data samples gathered on the \btsp sensor. These include motion tracking over known trajectories and their time-synchronized RGB images, force sensor readings for varying forces applied to the surface using different indenter diameters, and slippage data for several objects and their accompanying ground truth timestamps.

==> sections/math.tex <==
\graphicspath{{\subfix{../images/}}}

\section{Modelling of \btsp sensor}\label{sec:math}
In the following section, we present the mathematical formulations for a finite element model of the \btsp sensor, and how it characterizes the deformations of an ideal sensor. We then present an intuition as to how our proposed spatio-temporal gradient algorithm can approximate the finite element model at far lesser computational cost, on real hardware and data.

The finite element method provides the physical simulation of an ideal BioTac sensor and computes how applied forces on the skin results in some deformation of the skin's surfaces. These deformations are specific to certain parameters that dictate the nature of the materials being deformed, \ie they are physical properties of the BioTac sensor. A real \btsp sensor produces 24 taxel readings whose values are an indirect measurement of the deformation of the skin and underlying fluid. These values contain latent information about the change in volume of the skin for some given force. 

\subsection{Deformation Gradient in Continuum Mechanics}
\begin{figure}[ht!]
\centering
\begin{subfigure}[t]{0.4\linewidth}
    \includegraphics[height=0.9\linewidth]{images/biotac_deformation_desmos.pdf}
    \subcaption{Deformation of \btsp mesh due to applied force}
    \label{fig:deformation_nocolor}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[t]{0.4\linewidth}
    \includegraphics[height=0.9\linewidth]{images/biotac_deformations.png}
    \subcaption{Deformation correlated to applied force}
    \label{fig:deformation_color}
\end{subfigure}
\end{figure}

The deformation gradient is a fundamental measure of deformation of an object in continuum mechanics. It is a second order tensor that describes how an infinitesimally small segment of a surface (the material vector) transforms to a new configuration. We consider such a segment $dX$ in the undeformed configuration that transforms to $dx$, to be described by deformation gradient $F$.
Mathematically, this is given by
\begin{align}
    % & F_{i,j} = \sigma_{i,j} + \frac{\partial u_i}{\partial x_j} \\
    F_{i,j} = \frac{\partial x_i}{\partial X_j}\label{eq:def_grad}
\end{align}
\textit{Intuitively, the deformation gradient $F$ is an all-encompassing measure of the deformation of material elements. It quantifies both the 3D and 2D shape change of the material, as well as overall rotation.} 

Taking the concept of material deformation one step further, we introduce the determinant $J$ of the deformation gradient $F$, which is the \textbf{ratio of the deformed to the undeformed volumes}, for infinitesimal volume elements. This is given by
\begin{equation}
    J = det(F) = \frac{dV}{dV_o} \label{eq:jacobian}
\end{equation}
\textit{Intuitively, $J$ describes the change in volume from undeformed to deformed state, for some applied force.}

Lastly, we present a mathematical relation that links the stress (force per unit area), the strain (displacement per unit area), and the volume deformation:
\begin{equation}
    W = \frac{\mu}{2}(I_1 - 3) + \frac{(J-1)^2}{d}\label{eq:WJ}
\end{equation}
Here, $W$ refers to the strain, $J$ refers to the volume deformation due to some applied force, and $\mu$,$d$ are material properties of the sensor skin.

The aforementioned equations describe the deformation of a solid surface such as the BioTac sensor when a given force is applied. Narang \etal \cite{narang2021interpreting} used these equations in a finite element model to simulate forces on such an ideal BioTac sensor, and obtained deformations of the surface for various applied forces.
However, when dealing with real-world versions of these sensors, we do not have available to us the exact model of the surface or the deformation of said surface for some applied force. Instead, we leverage the inherent sensing mechanism of the \btsp sensor, which provides us with raw taxel values whose spatial coordinates and magnitudes correspond to the magnitude and location of the applied force on the surface.
\textit{In essence, the taxel values can be said to encode the approximate values of $W$ and $J$, as referred to in Eqn.~\ref{eq:WJ} above.}

\subsection{Motivation for Spatio-Temporal Gradients}
Owing to the physical design of the \btsp sensor, the raw tactile data that is generated when a tactile stimulus is applied to the skin contains latent information about the deformations and forces of said stimulus. However, this data is generated at discrete time intervals, which in case of the \btsp is around 0.01$s$ or a rate of 100 Hz.
Referring back to Eqns.~\ref{eq:def_grad} and \ref{eq:jacobian}, and consequently the results of Eq.~\ref{eq:WJ}, we see that they are all contingent upon infinitesimally small deformations and volume changes. In the case of finite element modelling, these equations are computed on an extremely small timestep, which is part of what makes the method computationally intensive and slow.

In our case, with the real-world \btsp, between two discrete data points obtained at 0.01$s$ intervals, the taxel values contain latent information about two deformation states of the sensor. However, there are in reality infinitely many intermediate deformations between these two states. The spatio-temporal gradients essentially interpolate these intermediate deformations, and their corresponding timestamps, and provide us with a detailed representation of how the surface volume deforms from one state to the next. One benefit of this approach is that due to the noise inherent to the sensing mechanism of the \btsp, the spatio-temporal interpolation can be tuned to reject all those intermediate changes that do not contribute to a significant deformation of the surface, thus keeping only those that are relevant. This has obvious noise-removal effects, as well as improving robustness when compared to raw tactile values.

==> sections/math_new.tex <==
\graphicspath{{\subfix{../images/}}}

\section{Modelling of \btsp sensor}\label{sec:math}
In the following section, we present the mathematical formulations for a finite element model of the \btsp sensor, and how it characterizes the deformations of an ideal sensor. We then present an intuition as to how our proposed spatio-temporal gradient algorithm can approximate the finite element model at far lesser computational cost, on real hardware and data.

The finite element method provides the physical simulation of an ideal BioTac sensor and computes how applied forces on the skin results in some deformation of the skin's surfaces. These deformations are specific to certain parameters that dictate the nature of the materials being deformed, \ie they are physical properties of the BioTac sensor. A real \btsp sensor produces 24 taxel readings whose values are an indirect measurement of the deformation of the skin and underlying fluid. These values contain latent information about the change in volume of the skin for some given force. 

\subsection{Deformation Gradient in Continuum Mechanics}
\begin{figure}[ht!]
\centering
\begin{subfigure}[t]{0.4\linewidth}
    \includegraphics[height=0.9\linewidth]{images/biotac_deformation_desmos.pdf}
    \subcaption{Deformation of \btsp mesh due to applied force}
    \label{fig:deformation_nocolor}
\end{subfigure}
\hspace{1em}
\begin{subfigure}[t]{0.4\linewidth}
    \includegraphics[height=0.9\linewidth]{images/biotac_deformations.png}
    \subcaption{Deformation correlated to applied force}
    \label{fig:deformation_color}
\end{subfigure}
\end{figure}

The deformation gradient is a fundamental measure of deformation of an object in continuum mechanics. It is a second order tensor that describes how an infinitesimally small segment of a surface (the material vector) transforms to a new configuration. We consider such a segment $dX$ in the undeformed configuration that transforms to $dx$, to be described by deformation gradient $F$.
Mathematically, this is given by
\begin{align}
    % & F_{i,j} = \sigma_{i,j} + \frac{\partial u_i}{\partial x_j} \\
    F_{i,j} = \frac{\partial x_i}{\partial X_j}\label{eq:def_grad}
\end{align}
\textit{Intuitively, the deformation gradient $F$ is an all-encompassing measure of the deformation of material elements. It quantifies both the 3D and 2D shape change of the material, as well as overall rotation.} 

Taking the concept of material deformation one step further, we introduce the determinant $J$ of the deformation gradient $F$, which is the \textbf{ratio of the deformed to the undeformed volumes}, for infinitesimal volume elements. This is given by
\begin{equation}
    J = det(F) = \frac{dV}{dV_o} \label{eq:jacobian}
\end{equation}
\textit{Intuitively, $J$ describes the change in volume from undeformed to deformed state, for some applied force.}

Lastly, we present a mathematical relation that links the stress (force per unit area), the strain (displacement per unit area), and the volume deformation:
\begin{equation}
    W = \frac{\mu}{2}(I_1 - 3) + \frac{(J-1)^2}{d}\label{eq:WJ}
\end{equation}
Here, $W$ refers to the strain, $J$ refers to the volume deformation due to some applied force, and $\mu$,$d$ are material properties of the sensor skin.

The aforementioned equations describe the deformation of a solid surface such as the BioTac sensor when a given force is applied. Narang \etal \cite{narang2021interpreting} used these equations in a finite element model to simulate forces on such an ideal BioTac sensor, and obtained deformations of the surface for various applied forces.
However, when dealing with real-world versions of these sensors, we do not have available to us the exact model of the surface or the deformation of said surface for some applied force. Instead, we leverage the inherent sensing mechanism of the \btsp sensor, which provides us with raw taxel values whose spatial coordinates and magnitudes correspond to the magnitude and location of the applied force on the surface.
\textit{In essence, the taxel values can be said to encode the approximate values of $W$ and $J$, as referred to in Eqn.~\ref{eq:WJ} above.}

\subsection{Motivation for Spatio-Temporal Gradients}
Owing to the physical design of the \btsp sensor, the raw tactile data that is generated when a tactile stimulus is applied to the skin contains latent information about the deformations and forces of said stimulus. However, this data is generated at discrete time intervals, which in case of the \btsp is around 0.01$s$ or a rate of 100 Hz.
Referring back to Eqns.~\ref{eq:def_grad} and \ref{eq:jacobian}, and consequently the results of Eq.~\ref{eq:WJ}, we see that they are all contingent upon infinitesimally small deformations and volume changes. In the case of finite element modelling, these equations are computed on an extremely small timestep, which is part of what makes the method computationally intensive and slow.

In our case, with the real-world \btsp, between two discrete data points obtained at 0.01$s$ intervals, the taxel values contain latent information about two deformation states of the sensor. However, there are in reality infinitely many intermediate deformations between these two states. The spatio-temporal gradients essentially interpolate these intermediate deformations, and their corresponding timestamps, and provide us with a detailed representation of how the surface volume deforms from one state to the next. One benefit of this approach is that due to the noise inherent to the sensing mechanism of the \btsp, the spatio-temporal interpolation can be tuned to reject all those intermediate changes that do not contribute to a significant deformation of the surface, thus keeping only those that are relevant. This has obvious noise-removal effects, as well as improving robustness when compared to raw tactile values.

==> sections/math_newnew.tex <==
\graphicspath{{\subfix{../images/}}}

\subsection{Motivation}
\label{subsec:motivation}
\chethan{Seems out of place, maybe put this in experiments}
We consider for our work the \btsp tactile sensor, which comes with a unique sensing mechanism as compared to other contemporary tactile sensors. Tactile sensing mechanisms, as they are available commercially today, lie on a spectrum ranging from \textit{accurate sensing capabilities} on one side to \textit{biomimetic form-factors} on the other. Most sensors on this spectrum make trade-offs on form factor to provide high accuracy. The \btsp is one particular sensor that strikes a right balance and is in the middle of the range, where we have a physical shape and sensing mechanism very close to the human finger tip, but this comes at the cost of accuracy and fidelity of sensing. 

\subsection{Challenges with Fluid-Conductive Sensors}
\label{subsec:challenges}
% Unlike optical-tactile, magnetic or capacitive tactile sensors, fluid based tactile sensors use a conductive fluid to transmit electrical impulses from four spatially distributed excitation electrodes to 24 sensing locations (taxels) distributed irregularly over a solid core. The values generated by the 24 taxels are thus primarily dependent on the characteristics of the fluid, specifically its conductivity.
Unlike optical-tactile, magnetic or capacitive tactile sensors, fluid based tactile sensors use a conductive fluid to transmit electrical impulses from spatially distributed excitation electrodes to a few sensing locations (taxels) distributed over a solid core. The values generated by the taxels are thus primarily dependent on the characteristics of the fluid, specifically its conductivity.\\
The conductivity of a fluid, such as the electrolytic solution present in the \btsp sensor is non-linearly related to various external factors. These include, but are not limited to the temperature of the fluid, the humidity of the surroundings, the area and distance between the excitation and sensing electrodes, and the concentration of the conductive fluid. Each of these factors contribute non-linearly \cite{wettels2008biomimetic} to the overall noise of each measurement at the respective taxel. Furthermore, the noise characteristics of the sensor electronics are also non-linear which further exacerbate the situation.\\
We also need to consider sources of noise in the electronic implementation of each taxel's sensing mechanism, which include amplification and analog-to-digital conversion circuitry among others.
\cornelia{Somewhere here or in the next section we need refer to the relation of volumetric deformation and taxel values, mentioned under Contribution 1}
\subsection{Modelling Fluid-Conductive Sensors}
\label{subsec:modelling}
While it might be feasible to model each of the aforementioned sources of noise independently and in isolation, the combination and interactions between them when considered together in the system makes it an arduous task. There have been several attempts to develop a physical model of the BioTac sensor, the most recent of which is presented in the work by Narang, \etal\cite{narang2021sim}. In this, the authors present a finite element model (FEM) of an ideal BioTac sensor, and provide an accurate simulation of the skin, the sensing core, and the internal fluid. While the FEM approach provides a physically accurate measurement of the deformation of the skin and fluid based on force stimuli, it does not account for the sources of noise described earlier. This is because the model of the sensor electronics are not considered along with the computational challenges of fluid modelling. Currently, to the best of our knowledge, there is no mathematical model between sensor readings and skin deformations, thereby inhibiting research in this area when utilizing raw sensor measurements.
% \nitin{We need to make a strong point of how we can avoid this}

\subsection{Bio-inspired motivation for logarithmic change}
\label{subsec:log-change}
In our work, we draw inspiration from nature regarding how one uses tactile data, developing an ``inuition'' based on how changes over the skin surfaces are related to location of touch and relative forces. To this end, we break away from the core robotics ideology that one requires a complex and accurate mathematical model or a very high quality sensor to perform useful tasks. In particular, we are driven by nature's efficient and parsimonious implementations which perform amazingly well with minimal quality sensors and very simple computing. 

% We take a  different approach in our proposed work. If we proceed with the assumption that the \btsp is useful as a tool for measuring tactile stimulus, namely the location of touch and relative forces, 


% we hypothesize that neither the accurate simulation of the sensor nor the complex noise interactions are necessary to perform useful experiments and tasks with the sensor. 

To build such an efficient data representation for fluid based sensors, we look at the Weber-Fechner Laws, which states that the perceived stimulus on any of the human senses is related via an exponential function to the actual stimulus. As a result, humans perceive stimuli such as touch, sound or light as the changes in the logarithm between existing values and new ones.
It is thus not surprising that the manufacturers of the \btsp sensor, who designed it to be as anthropomorphic as possible, also recommend that the best way to process the data from their sensors is to use relative changes instead of raw taxel values.
% \nitin{Figure out a better way to say this and till end of this section: This idea is reinforced by the manufacturers of the \btsp, who also recommend not using raw taxel values from the sensor, but instead using changes between consecutive taxel data.}
In practice, the two main challenges with the \btsp sensor are that
\begin{enumerate*}
  \item the different taxels do not have same baseline value, and
  \item the taxel values exhibit a low signal to noise ratio.
\end{enumerate*}
By computing only the taxel changes on a logarithmic scale, our values become independent of the baseline and are more robust to noise, thus tackling both aforementioned issues.

\subsection{Computing events from raw data}
\label{subsec:computing-events}
We consider two consecutive packets of taxel data, at times $t$ and $t+\delta$ respectively. Each of these packets contain the raw taxel values $X^{t}_{k=1\dots24}$ and $X^{t+\delta}_{k=1\dots24}$. We then compute the logarithmic change between each of the $j \in {1, 24}$  consecutive taxels, and fire an event when  the logarithm of the value at the taxel increases or decreases by a threshold value $\tau$. That is, when: 
\vspace{-3px}
\begin{equation}
| \ln X^{t= i + \delta}_{j} - \ln X^{t= i}_{j} | > \tau
\end{equation}
\vspace{-12px}\\
In other words, a positive event is ``fired'' when 
\vspace{-3px}
\begin{equation}
\ln X^{t= i + \delta}_{j} > e^{\tau}\ln X^{t= i}_{j}
\end{equation}
\vspace{-12px}\\
and a negative event when 
\vspace{-3px}
\begin{equation}
\ln X^{t= i}_{j} > e^{\tau}\ln X^{t= i+ \delta}_{j}
\end{equation}
\vspace{-12px}\\
This gives us intermediate taxel values between times $t$ and $t +\delta$, and their respective timestamps.

We know from the design of the sensor, as well as ideal sensor simulations that the largest change in the values of the taxels correlates with the region of highest tactile stimulus. Also, this change is dependent on the forces already present on the region of touch, and reaches saturation and demonstrates hysteresis in the raw values. Our algorithm accounts for that by non-linearly interpolating the taxel data, on the log scale.
The previously obtained taxel events thus give us a temporal gradient over the change in taxel values, caused by the deformation of the skin and fluid because of the applied force stimulus. Intuitively, these intermediate events between two discrete taxel data values signifies change in localized volume of the skin and fluid over time because of the applied tactile stimulus.

As part of our algorithm, we then process these spatially discrete events for each of the 24 taxel locations and convert them into a continuous, interpolated surface. We use a Voronoi tesselation of the discrete and irregular grid, and perform Natural Neighbors Interpolation to construct an event surface, that gives us an interpolated event value at each point. This surface indirectly depicts the deformation of the skin and fluid, due to applied stimulus. Since the deformation due to applied forces on the \btsp is greatest at the region of touch, we generate iso-contours of the event surface, and consider only the maximal valued contour as the region of touch.
